Genome assembly, from practice to theory: safe, complete and linear-time

Genome assembly asks to reconstruct an unknown string from many shorter substrings of it. Even though it is one of the key problems in Bioinformatics, it is generally lacking major theoretical advances. Its hardness stems both from practical issues (size and errors of real data), and from the fact that problem formulations inherently admit multiple solutions. Given these, at their core, most state-of-the-art assemblers are based on finding non-branching paths (unitigs) in an assembly graph. If one defines a genome assembly solution as a closed arc-covering walk of the graph, then unitigs appear in all solutions, being thus safe partial solutions. All all such safe walks were recently characterized as omnitigs, leading to the first safe and complete genome assembly algorithm. Even if omnitig finding was improved to quadratic time, it remained open whether the crucial linear-time feature of finding unitigs can be attained with omnitigs. We describe a surprising $O(m)$-time algorithm to identify all maximal omnitigs of a graph with $n$ nodes and $m$ arcs, notwithstanding the existence of families of graphs with $\Theta(mn)$ total maximal omnitig size. This is based on the discovery of a family of walks (macrotigs) with the property that all the non-trivial omnitigs are univocal extensions of subwalks of a macrotig, with two consequences: (1) A linear-time output-sensitive algorithm enumerating all maximal omnitigs. (2) A compact $O(m)$ representation of all maximal omnitigs, which allows, e.g., for $O(m)$-time computation of various statistics on them. Our results close a long-standing theoretical question inspired by practical genome assemblers, originating with the use of unitigs in 1995. We envision our results to be at the core of a reverse transfer from theory to practical and complete genome assembly programs, as has been the case for other key Bioinformatics problems.

==> arxiv 2/micromacro.tex <==
\section{Macronodes and macrotigs}
\label{sec:macronode-macrotigs}

In this section, unless otherwise stated, we assume that the input graph is \emph{compressed}, in the sense that it has no biunivocal nodes and arcs. In some algorithms we will also require that the graph has constant in- and out-degree. In \Cref{sec:prepro} we show how these properties can be guaranteed, by transforming any strongly connected graph $G$ with $m$ arcs, in time $O(m)$, into a compressed graph of constant degree and with $O(m)$ nodes and arcs. 

In a compressed graph all arcs are split, join or bivalent. Moreover, in compressed graphs, the following observation holds.
% (see \Cref{fig:obsbiv} in \Cref{app:addfig}, for an example).

%\begin{figure}[htb]
%	\centering
%	\includegraphics[scale=0.9]{la_figures/la_fig-obs-biv2.pdf}
%	\caption{
%		Let $f$ be a join arc and $g$ be a split arc, in a compressed graph. Left: $W$ is represented as the dotted path from $h(f)$ to $t(g)$, where $u$ is a bivalent node.
%		Right: $W$ is the dotted path from $h(f)$ to $t(g)$, where $b \in W$ is a bivalent arc.
%	}
%	\label{fig:obsbiv}
%\end{figure}

\begin{observation}
\label{obs:joinsplitarcs}
	Let $G$ be a compressed graph. Let $f$ and $g$ be a join and a split arc, respectively, in $G$. The following holds:
	\begin{itemize}
	\itemsep0em
	\item[$(i)$] if $fWg$ is a walk, then $W$ has an internal node which is a bivalent node;
	\item[$(ii)$] if $gWf$ is a walk, then $gWf$ contains a bivalent arc.
	\end{itemize}
\end{observation}

In the rest of this paper we will use the following technical lemmas (omitted proofs are in \Cref{subsec:compression}.).

\begin{restatable}{lemma}{omnitigbivnodearc}
\label{lem:omnitig-biv-node-arc}
Every maximal omnitig of a compressed graph contains both a join arc and a split arc.
Moreover, it has a bivalent arc or an internal bivalent node.
\end{restatable}

\vspace{-.3cm}
\begin{restatable}{lemma}{noftwice}
\label{lem:noftwice}
Let $e$ be a join or a split arc. No omnitig can traverse $e$ twice.
\end{restatable}

\vspace{-.3cm}
\begin{restatable}{lemma}{nobivntwice}
\label{lem:nobivntwice}
Let $u$ be a bivalent node. No omnitig contains $u$ twice as an internal node.  
\end{restatable}

\subsection{Macronodes}

We now introduce a natural partition of the nodes of a compressed graph; each class of such a partition (i.e. a \emph{macronode}) contains precisely one bivalent node. We identify each class with the unique bivalent node they contain. All other nodes belonging to the same class are those that either reach the bivalent node with a join-free path or those that are reached by the bivalent node with a split-free path (recall \Cref{fig:macronodes-example}). 

\begin{definition}[Macronode]
	\label{def:macronode}
	Let $v$ be a bivalent node of $G$. Consider the following sets:
	\begin{itemize}
		\itemsep0em
		\item[] $R^+(v) := \{ u \in V(G) : \exists~ \text{a join-free path from}~ v ~\text{to}~ u \}$;
		\item[] $R^-(v) := \{ u \in V(G) : \exists~ \text{a split-free path from}~ u ~\text{to}~ v \}.$ 
	\end{itemize} 
	The subgraph $\macronode{v}$ induced by $R^+(v)\cup R^-(v)$ is called the \emph{macronode centered in $v$}.
\end{definition}


\begin{restatable}{lemma}{macropartition}
\label{obs:macropartition}
In a compressed graph $G$, the following properties hold:
\begin{itemize}
	\itemsep0em
    \item[i)] The set $\{V(\macronode{v}) : \text{$v$ is a bivalent node of $G$}\}$ is a partition of $V(G)$. 
    \item[ii)] In a macronode $\mathcal{M}_v$, $R^+(v)$ and $R^-(v)$ induce two trees with common root $v$, but oriented in opposite directions. Except for the common root, the two trees are node disjoint, all nodes in $R^-(v)$ being join nodes and all nodes in $R^+(v)$ being split nodes.
    \item[iii)] The only arcs with endpoints in two different macronodes are bivalent arcs. 
\end{itemize}
%Notice that, given any bivalent arc $b$, the endpoints of its univocal extension $U(b)$ are bivalent nodes, i.e., are centers of two macronodes, which may be the same node, or different nodes (see \Cref{fig:macronodes-A} in the appendix).
\end{restatable}

To analyze how omnitigs can traverse a macronode and the degrees of freedom they have in choosing their directions within the macronode, we introduce the following definitions. \emph{Central-micro omnitigs} are the smallest omnitigs that cross the center of a macronode. \emph{Left- and right-micro omnitigs} start from a central-micro omnitig and proceed to the periphery of a macronode. Finally, we combine left- and right-micro omnitigs into microtigs (which are not necessarily omnitigs themselves); recall \Cref{fig:microtigs}.

\begin{definition}[Micro omnitigs, microtigs]
\label{def:omni_type}
Let $f$ be a join arc and $g$ be a split arc, such that $fg$ is an omnitig.
\begin{itemize}
\itemsep0em
\item The omnitig $fg$ is called a \emph{central-micro omnitig}.
\item An omnitig $fgW$ ($Wfg$, resp.) that does not contain a bivalent arc as an internal arc is called a \emph{right-micro omnitig} (respectively, \emph{left-micro omnitig}). 
\item A walk $W = W_1 fg W_2$, where $W_1 fg$ and $fg W_2$ are, respectively, a left-micro omnitig, and a right-micro omnitig, is called a \emph{microtig}.
\end{itemize}
\end{definition}

\begin{sloppypar}
Given a join arc $f$, we first find central micro-omnitigs (of the type $fg$) with the generic function $\mathsf{RightExtension}(G,f,W)$ from \Cref{alg:extensions}, where $W$ is a join-free path (possibly empty). This extension uses the following weak version of the \extprop (since $W$ is join-free). To build up the intuition, we also give a self-contained proof of this weaker result.
\end{sloppypar}

\begin{lemma}[Weak form of the \extprop~ (\Cref{thm:strong-ita-result})]
\label{lem:weak_ita_lem}
Let $fW$ be an omnitig in $G$, where $f$ is a join arc and $W$ is a join-free path. 
Then $fWg$ is an omnitig if and only if $g$ is the only arc with $t(g) = h(W)$ such that there exists a path from $h(g)$ to $h(f)$ in $G \smallsetminus f$.
\end{lemma}
\begin{proof}
To prove the existence of an arc $g$, which satisfies the condition, consider any closed path $Pf'$ in $G$, where $f'$ is an arbitrary sibling join arc of $f$. 
Notice that $W$ is a prefix of $Pf'$, since $fW$ is an omnitig, since otherwise one can easily find a forbidden path for the omnitig $fW$ as a subpath of $Pf'$, from the head of the very first arc of $Pf'$ that is not in $W$ to $h(f')$. Therefore, let $g$ be the the first arc of $Pf'$ after the prefix $W$, in such a way that the suffix of $Pf'$ starting from $h(g)$ is a path to $h(f)$ in $G \smallsetminus f$.

For the direct implication, assume that there is a path $P$ in $G \smallsetminus f$ from $h(g')$, where $g'$ sibling of $g$ and $g' \neq g$, to $h(f)$. Then, this forbidden path $P$ contradicts the fact that $fWg$ is an omnitig.

For the reverse implication, assume that $fWg$ is not an omnitig. Then take any forbidden path $P$ for $fWg$. Since $fW$ is an omnitig, $P$ must start with some $g'$ sibling arc of $g, g' \neq g$. Since $W$ is join-free, then $P$ must end in $h(f)$ with the last arc different from $f$. Therefore, $P$ is a path from $h(g')$ to $h(f)$ in $G \smallsetminus f$.
\end{proof}

Not only \Cref{lem:weak_ita_lem} gives us an efficient extension mechanism, but it also immediately implies the \yintprop (for clarity of reusability, we state both its symmetric variants). 

\begin{corollary}[\yintprop]
\label{cor:Y-lemma}
Let $fWg$ be an omnitig, where $f$ is a join arc, and $g$ is a split arc.
\begin{itemize}
	\itemsep0em
    \item[i)] If $W$ is a join-free path (possibly empty), then for any $g'$ a sibling split arc of $g$, the walk $fWg'$ is not an omnitig.
    \item[ii)] If $W$ is a split-free path (possibly empty), then for any $f'$ a sibling join arc of $f$, the walk $f'Wg$ is not an omnitig.
\end{itemize}
\end{corollary}

We now use the \yintprop to prove the \xintprop.

\begin{proof}[Proof of the \xintprop~(\Cref{thm:Xthm})]
For point $i)$, assume there exists an arc $g_3$, distinct from $g_1$ and $g_2$, such that $t(g_3) = v$. Consider any shortest closed path $g_3 P$ (with $P$ possibly empty), which exists by the strong connectivity of $G$. Let $f$ be the last arc of $P$.
If $f \neq f_1$ then $g_3P$ is a forbidden path for the omnitig $f_1 g_1$, since $g_3 \neq g_1$.
Otherwise, if $f = f_1$ then $g_3 P$ is a forbidden path for the omnitig $f_2 g_2$, since $g_3 \neq g_1$.
In both cases we reached a contradiction, therefore $g_1$ and $g_2$ are the only arcs in $G$ with $t(g_1) = t(g_2) = v$. 
To prove that $f_1$ and $f_2$ are the only arcs in $G$ with $h(f_1) = h(f_2) = v$ one can proceed by symmetry.
 
Point $ii)$ follows from \Cref{cor:Y-lemma} (by taking the $W$ path of its statement to be empty) and from the symmetric analogue of \Cref{cor:Y-lemma}.
\end{proof}

\begin{sloppypar}
Given an omnitig $fg$, we obtain the maximal right-micro omnitig with function $\mathsf{MaximalRightMicroOmnitig}(G,f,g)$ from \Cref{alg:extensions}. This works by extending $fg$, as much as possible, with the function $\mathsf{RightExtension}(G,f,W)$ (where initially $W = g$). This extension stops when reaching the periphery of the macronode (i.e.~a bivalent arc).
\end{sloppypar}

\begin{algorithm}[t]
    \caption{Functions $\mathsf{RightExtension}$ and $\mathsf{MaximalRightMicroOmnitig}$.}
    \label{alg:extensions}
    \Function{$\mathsf{RightExtension}(G,f,W)$}{
	    \Input{The compressed graph $G$, $fW$ omnitig with $W$ join-free.}
	    \Returns{The unique arc $e$ such that $fWe$ is an omnitig, if it exists. Otherwise, $\Nil$.}
		\BlankLine
		
		$S \gets \{ e \in E(G) \mid t(e) = h(W) \text{ and there is a path from } h(e) \text{ to } h(f) \text{ in } G \smallsetminus f \}$ \;
		
		\lIf{there is exactly one arc $e \in S$}{\Return $e$}
		
    	\BlankLine

		\Return $\Nil$ \;
	}
	\BlankLine
	\Function{$\mathsf{MaximalRightMicroOmnitig}(G,f,g)$}{
		\Input{The compressed graph $G$, $fg$ omnitig with $f$ join arc and $g$ split arc.}
		\Returns{The path $W$ such that $fgW$ is a maximal right-micro omnitig.}
		
    	\BlankLine

        $W \gets$ empty path

	    \While{\True}{
    	    \lIf{$fgW$ ends with a bivalent arc}{\Return $W$}
    
    	    $e \gets \mathsf{RightExtension}(G,f,W)$ \;
    	    \lIf{$e = \Nil$}{\Return $W$}

        	\BlankLine

            $W \gets We$ \;
	    }
    }
\end{algorithm}

\begin{lemma}
\label{lem:alg1correct}
The functions in \Cref{alg:extensions} are correct. Moreover, assuming that the graph has constant degree, we can preprocess it in time $O(m+n)$ time, so that $\mathsf{RightExtension}(G,f,W)$ runs in constant time, and $\mathsf{MaximalRightMicroOmnitig}(G,f,g)$ runs in time linear in its output size.
\end{lemma}
\begin{proof}
For $\mathsf{RightExtension}(G,f,W)$, recall \Cref{lem:weak_ita_lem} and \Cref{cor:italiano_result} and that the input graph is a compressed graph, and as such every node has constant degree.

For $\mathsf{MaximalRightMicroOmnitig}(G,f,g)$, notice that every iteration of the \emph{while} loop increases the output by one arc and takes constant time, since $\mathsf{RightExtension}(G,f,W)$ runs in $O(1)$ time.
\end{proof}

\Cref{alg:maximalbigenerator} is the procedure to obtain all maximal microtigs of a compressed graph. It first finds all central micro-omnitigs $fg$ (with $\mathsf{RightExtension}(G,f,\emptyset)$), and it extends each to the right (i.e.~forward in $G$) and to the left (i.e.~forward in $G^R$) with $\mathsf{MaximalRightMicroOmnitig}$.

\begin{algorithm}[htb]
    \caption{Function $\mathsf{AllMaximalMicrotigs}$
    \label{alg:maximalbigenerator}}
    
    \Function{$\mathsf{AllMaximalMicrotigs}(G)$}{
		\Input{The compressed graph $G$.}
		\Returns{All the maximal microtigs in $G$.}
		
    	\BlankLine
    	
		$S \gets \emptyset$ \;
		
		\ForEach{bivalent node $u$ in $G$}{
    		\ForEach{join arc $f$ with $h(f) = u$}{
        		\ForEach{split arc $g$ with $t(g) = u$}{
        		    \If{$g = \mathsf{RightExtension}(G,f,\emptyset)$\label{line:right-extension-check}}{
                	    \Comment{$fg$ is a central-micro omnitig}

                        \BlankLine
                	    
                	    \Comment{applied symmetrically for left- and right-micro omnitigs}

                	    $W_1 \gets \mathsf{MaximalRightMicroOmnitig}(G^R,g,f)$ \;
                	    $W_2 \gets \mathsf{MaximalRightMicroOmnitig}(G,f,g)$ \;
                	    
                        \BlankLine

                        \BlankLine

                	    add $W_1 fg W_2$ to $S$ \;
        		    }
    		    }
		    }
		}
		
    	\BlankLine
    	
    	\Return $S$ \;
    }
\end{algorithm}

To prove the correctness of \Cref{alg:maximalbigenerator}, we need to show some structural properties of micro-omnitigs and microtigs, as follows.

\begin{lemma}
\label{lem:atmostonemicro}
Let $fg$ be a central-micro omnitig. The following hold:
\begin{itemize}
	\itemsep0em
    \item[i)] There exists at most one maximal right-micro omnitig $fgW$, and at most one maximal left-micro omnitig $Wfg$.
    \item[ii)] There exists a unique maximal microtig containing $fg$.
\end{itemize}
\end{lemma}
\begin{proof}
We prove only the first of the two symmetric statements in $i)$. If $g$ is a bivalent arc, the claim trivially holds by definition of maximal right-micro omnitig. Otherwise, a minimal counterexample consists of two right-micro omnitigs $fgPg_1$ and $fgPg_2$ (with $P$ a join-free path possibly empty), with $g_1$ and $g_2$ distinct sibling split arcs.  
Since $gP$ is a join-free path, the fact that both $fgPg_1$ $fgPg_2$ are omnitigs contradicts the \yintprop (\Cref{cor:Y-lemma}).
%$g_1$ is the only arc with $t(g_1) = h(P)$, such that there exists a path from $h(g_1)$ to $h(f)$ in $G \smallsetminus f$. Thus, $fgPg_2$ is not an omnitig, a contradiction.

For $ii)$, given $fg$, by $i)$ there exists at most one maximal left-micro omnitig $W_1fg$ and at most one maximal right-micro omnitig $fgW_2$, as such there is at most one maximal microtig $W_1 fg W_2$. 
%\alex{Elia}: Use the first bullet and the previous: "For any join arc $f$, there exists at most one central-micro omnitig $fg^\ast$, where $g^\ast$ is a split arc, with $t(g^\ast) = h(f)$. Symmetrically, for any split arc $g$, there exists at most one central-micro omnitig $f^\ast g$, where $f^\ast$ is a join arc, with $h(f^\ast) = t(g)$."
\end{proof}

\begin{comment}
\begin{lemma}
\label{lem:unique_rightgen-f}
For any join arc $f$, there exists at most one maximal right-micro omnitig $fgW$. For any split arc $g$ there exists at most one maximal left-micro omnitig $Wfg$.
\end{lemma}
\begin{proof}
We prove only the first of the two symmetric statements.
A minimal counterexample is the existence of two right-micro omnitigs $fPg$ and $fPg'$ (with $P$ possibly empty), with $g$ and $g'$ distinct sibling split arcs. 
Notice that, by \Cref{lem:weak_ita_lem}, $g$ is the only arc with $t(g) = h(P)$, such that there exists a path from $h(g)$ to $h(f)$ in $G \smallsetminus f$, as such $fPg'$ is not an omnitig, a contradiction.
\end{proof}

\begin{lemma}
\label{cor:unique-big}
Every central-micro omnitig $fg$ is contained in a unique maximal microtig.
\end{lemma}

\begin{proof}
\alex{Elia}: Use \Cref{lem:unique_rightgen-f} and the previous corollary: For any join arc $f$, there exists at most one central-micro omnitig $fg^\ast$, where $g^\ast$ is a split arc, with $t(g^\ast) = h(f)$. Symmetrically, for any split arc $g$, there exists at most one central-micro omnitig $f^\ast g$, where $f^\ast$ is a join arc, with $h(f^\ast) = t(g)$.
\end{proof}

\begin{lemma}
\label{lem:uniquearcbig}
For any arc $e$, there exists at most one maximal microtig of the form $W_1 fg W_2$, with $fg$ central-micro omnitig and $e \in W_1f$, and at most one maximal microtig of the form $W_1 fg W_2$, with $fg$ is a central-micro omnitig and $e \in g W_2$.
\end{lemma}
\begin{proof}
We need to prove only the first of the two symmetric statements.
Consider a central-micro omnitig $fg$ and an microtig $W_1 fg W_2$, with $e \in W_1f$; as such, $e$ is a join arc. Hence, consider the unique split-free path $P$ from $h(e)$ to a bivalent node $u$. Notice that $f$ is uniquely defined as the last arc of $P$. By \Cref{lem:unique_rightgen-f} and its corollaries, there exists a unique maximal microtig that contains $fg$. 
\end{proof}
\end{comment}

\begin{lemma}
\label{lem:arcs-in-microtigs}
Let $e$ be an arc. The following hold:
\begin{itemize}
	\itemsep0em
    \item[i)] if $e$ is not a bivalent arc, then there exists at most one maximal microtig containing~$e$.
    \item[ii)] if $e$ is a bivalent arc, there exist at most two maximal microtigs containing~$e$, of which at most one is of the form $eW_1$, and at most one is of the form $W_2e$.
\end{itemize}
\end{lemma}
\begin{proof}
By symmetry, in $i)$ we only prove the case in which $e$ is a split-free arc. Notice that by \Cref{obs:macropartition}, $h(e)$ belongs to a uniquely determined macronode $\macronode{u}$ of $G$; let $P$ be the split-free path in $G$, from $h(e)$ to $u$. Let $f$ be the last arc of $eP$ ($f = e$ if $P$ is empty). By the \xintprop (\Cref{thm:Xthm}), there exists at most one split arc $g$ with $t(g) = u = h(f)$ such that $fg$ is an omnitig; if it exists, $fg$ is a central-micro omnitig, hence by \Cref{lem:atmostonemicro}, there is at most one maximal left-micro omnitig $Wfg$. Finally, if such a maximal left-micro omnitig exists, $ePg$ is a subwalk of $Wfg$, by the \yintprop (\Cref{cor:Y-lemma}). Otherwise, a minimal counterexample consists of paths $f_1 R g$ (subpath of $ePg$) and $f_2 R g$ (subpath of $Wfg$), where $f_1 \neq f_2$ and $R$ is a split-free path, since it is subpath of the split-free path $eP$; since both $f_1 R g$ and $f_2 R g$ are omnitigs, this contradicts the \yintprop.

For $ii)$, we again prove only one of the symmetric cases. The proof is identical to the above, since by \Cref{obs:macropartition}, $h(e)$ belongs to a unique macronode $\macronode{v_1}$ of $G$. As such, $e$ belongs to at most one maximal microtig $eW_1$ in $\macronode{v_1}$. Symmetrically, $t(e)$ belongs to a uniquely determined macronode $\macronode{v_2}$ of $G$. Thus, $e$ belongs to at most one maximal microtig $W_2e$ within $\macronode{v_2}$. 
\end{proof}

\begin{theorem}[Maximal microtigs]
\label{lem:maximalbigenerator}
The maximal microtigs of any strongly connected graph $G$ with $n$ nodes, $m$ arcs, and arbitrary degree have total length $O(n)$, and can be computed in time $O(m)$, with \Cref{alg:maximalbigenerator}.
\end{theorem}
\begin{proof}
First we prove the $O(n)$ bound on the total length. As we explain in \Cref{sec:prepro} we can transform $G$ into a compressed graph $G'$ such that $G'$ has $n' \leq n$ nodes and $m' \leq m$ arcs. 

Since $G'$ has at most $n'$ macronodes (recall that macronodes partition the vertex set, \Cref{obs:macropartition}), and every macronode has at most two maximal microtigs, then number of maximal microtigs is at most $2n'$. The total length of all maximal microtigs is bounded as follows. Every internal arc of a maximal microtig is not a bivalent arc, by definition. Since every non-bivalent arc appears in at most one maximal microtig (\Cref{lem:arcs-in-microtigs}), and there are at most $n'$ non-bivalent arcs in any graph with $n'$ nodes, then the number of internal arcs in all maximal microtigs is at most $n'$. Summing up for each maximal microtigs its two non-internal arcs (i.e., its first and last arc), we obtain that the total length of all maximal microtigs is at most $2n' + n' = 3n'$, thus $O(n)$.

As mentioned, in \Cref{sec:prepro} we show how to transform $G$ into a compressed graph $G'$ with $O(m)$ arcs, $O(m)$ nodes, and constant degree. On this graph we can apply \Cref{alg:maximalbigenerator}. Since every node of the graph has constant degree, the \emph{if} check in \Cref{line:right-extension-check} runs a number of times linear in the size $O(m)$ of the graph. Checking the condition in \Cref{line:right-extension-check} takes constant time, by \Cref{lem:alg1correct}; in addition, the condition is true for every central-micro omnitig $fg$ of the graph.
The \emph{then} block computes a maximal microtig and takes linear time in its size, \Cref{lem:alg1correct}. By \Cref{lem:arcs-in-microtigs} we find every microtig in linear total time.
\end{proof}

\subsection{Macrotigs}

In this section we analyze how omnitigs go from one macronode to another. Macronodes are connected with each other by bivalent arcs (\Cref{obs:macropartition}), but merging microtigs on all possible bivalent arcs may create too complicated structures. However, this can be avoided by a simple classification of bivalent arcs: those that connect a macronode with itself (\emph{self-bivalent}) and those that connect two different macronodes (\emph{cross-bivalent}), recall \Cref{fig:macronodes}.

\begin{definition}[Self-bivalent and cross-bivalent arcs]
A bivalent arc $b$ is called a \emph{self-bivalent arc} if $U(b)$ goes from a bivalent node to itself. Otherwise it is called a \emph{cross-bivalent arc}.
\end{definition}

A macrotig is now obtained by merging those microtigs from different macronodes which overlap only on a cross-bivalent arc, see also \Cref{fig:macrotig-example}.

\begin{definition}[Macrotig]
\label{def:macrotig}
Let $W$ be any walk. 
$W$ is called a \emph{macrotig} if 
\begin{enumerate}
	\itemsep0em
    %\item $W = b$ is a single bivalent arc, or 
    \item $W$ is an microtig, or
    \item By writing $W = W_0 b_1 W_1 b_2 \ldots b_{k-1} W_{k-1} b_k W_k$, where $b_1, \ldots, b_k$ are all the internal bivalent arcs of $W$, the following conditions hold:
    \begin{enumerate}
        \item the arcs $b_1, \ldots, b_k$ are all cross-bivalent arcs, and
        \item $W_0 b_1,\; b_1 W_1 b_2,\; \ldots,\; b_{k-1} W_{k-1} b_k,\; b_k W_k$ are all microtigs.
    \end{enumerate} 
\end{enumerate}
\end{definition}

Notice that the above definition does not explicitly forbid two different macrotigs of the form $W_0 b W_1$ and $W_0 b W_2$. However,  \Cref{lem:arcs-in-microtigs} shows that there cannot be two different microtigs $bW_1$ and $bW_2$, thus we immediately obtain:

\begin{lemma}
\label{lem:uniqueprotomni}
For any macrotig $W$ there exists a unique maximal macrotig containing $W$.
\end{lemma}
\begin{proof}
W.l.o.g.,~a minimal counterexample consists of a non-right-maximal macrotig $Wb$, such that there exist two distinct microtigs $bW_1$ and $bW_2$ (notice that $b$ is a cross-bivalent arc). By \Cref{lem:arcs-in-microtigs} applied to $b$, we obtain $bW_1 = bW_2$, a contradiction.
\end{proof}

The macrotig definition also does not forbid a cross-bivalent arc to be used twice inside a macrotig. In \Cref{lem:noetwiceinproto} below we prove that also this is not possible, using the following result.

 \begin{lemma}[\cite{DBLP:journals/talg/CairoMART19}]
\label{lem:acyclic}
For any two distinct non-sibling split arcs $g, g'$, write $g \prec g'$ if there exists an omnitig $g P g'$ where $P$ is split-free. Then, the relation $\prec$ is acyclic.
\end{lemma}


\begin{figure}[t]
	\centering
	\includegraphics[width=\textwidth]{la_figures/macrotigs-example.pdf}
\caption{\small Three macronodes $\mathcal{M}_{u},\mathcal{M}_{v},\mathcal{M}_{w}$ (as gray areas) with arcs color-coded as in \Cref{fig:macronodes-example}. Black walks mark their five maximal microtigs: $b_1 g_1\dots b_2$, $b_i\dots f_ig_i\dots b_{i+1}$ ($i \in \{2,3,4\}$), $b_5\dots f_5g_5$ ($g_5 = b_1$). The maximal macrotig $M$ is obtained by overlapping them on the cross-bivalent arcs $b_2,b_3,b_4,b_5$, i.e.~$M = b_1\dots b_2 \dots b_3\dots b_4\dots b_5 \dots b_1$. Notice that no arc is contained twice, with the exception of the cross-bivalent arc $b_1$, appearing as the first and last arc of $M$ (\Cref{lem:noetwiceinproto}). Bivalent nodes (e.g.~$u,v$) can appear (at most) twice in $M$ (by the \xintprop and \Cref{lem:atmostonemicro}).
\label{fig:macrotig-example}}
\end{figure}

\begin{lemma}
\label{lem:noetwiceinproto}
Let $W$ be a macrotig and let $e$ be an arc of $W$. If $e$ is self-bivalent, then $e$ appears at most twice in $W$ (as first or as last arc of $W$). Otherwise, $e$ appears only once.
% A macrotig $W$ does not contain an arc $e$ twice, unless $e$ is a self-bivalent arc.
\end{lemma}
\begin{proof}
If $e$ is self-bivalent, then \Cref{def:macrotig} implies that $e$ is either the first arc of $W$, the last arc of $W$, or both. Thus, $e$ appears at most twice.

Suppose now that $e$ is not self-bivalent. We first consider the case when $e$ is a split arc. We are going to prove that between any two consecutive non-self-bivalent split arcs the relation $\prec$ from \Cref{lem:acyclic} holds. Indeed, let $g$ and $g'$ be two consecutive (i.e.~closest distinct) non-self-bivalent split arcs along $W$: that is $gPg'$ subwalk of $W$, with $P$ a split-free path. Notice that $g$ and $g'$ are not sibling arcs; since otherwise, $g$ is a self-bivalent arc, by \Cref{obs:joinsplitarcs}. If $t(g')$ is not a bivalent node, then $P$ is empty. In this case, $g$ is a join-free arc, so $gg'$ is an omnitig; as such, $g \prec g'$.
Otherwise, if $t(g')$ is a bivalent node, then $gPg'$ is a left-micro omnitig and so it is an omnitig; as such, again, $g \prec g'$.

Suppose for a contradiction that $e$ is traversed twice. Since there are no internal self-bivalent arcs (as argued at the beginning of the proof), this would result in a cycle in the relation $\prec$, which contradicts \Cref{lem:acyclic}.

When $e$ is a non-self-bivalent join arc, we proceed symmetrically. First, notice that the relation defined in \Cref{lem:acyclic} is symmetric: if $f$ and $f'$ are two distinct non-sibling join arcs such that $fPf'$, with $P$ a join-free path, then $f \prec f'$. The claim above can be symmetrically adapted to hold for any two closest distinct non-self-bivalent join arcs $f$ and $f'$ within a macrotig (i.e.~corresponding to a subwalk of $W$ of the form $fPf'$, with $P$ a join-free path). Moreover, $f$ and $f'$ are not siblings; since otherwise, $f'$ is a self-bivalent arc, by \Cref{obs:joinsplitarcs}.    

Hence, by the acyclicity property of the relation $\prec$ on the reverse graph, the claim also holds for non-self-bivalent join arcs.
\end{proof}

Therefore, we can construct all \emph{maximal} macrotigs by repeatedly joining microtigs overlapping on cross-bivalent arcs, as long as possible, as in \Cref{alg:maxproto}. 

\begin{algorithm}[tb]
    \caption{Function $\mathsf{AllMaximalMacrotigs}$.}
	\label{alg:maxproto}
	
	\Function{$\mathsf{AllMaximalMacrotigs}(G)$}{
		\Input{The compressed graph $G$.}
		\Returns{All the maximal macrotigs in $G$.}
		
    	\BlankLine
    	
		$S \gets \mathsf{AllMaximalMicrotigs}(G)$ \;
		
		\While{$\exists$ $W_1 b \in S$ \And $b W_2 \in S$ with $b$ cross-bivalent arc \And non-empty $W_1, W_2$}{
		    remove $W_1 b$ and $b W_2$ from $S$ \;
		    add $W_1 b W_2$ to $S$ \;
		}
		
    	\BlankLine
    	
    	\Return $S$ \;
    }
\end{algorithm}



%\begin{corollary}\label{cor:protoinmaxiproto}
%Every macrotig is a subwalk of a maximal macrotig.
%\end{corollary}


%
%    \begin{lemma}
%    \label{lem:arcs-in-macrotigs}
%    % \label{cor:max2protoforbiv}
%    % \label{cor:uniqueprotoforarcint}
%    \alex{Move this inside the proof of \Cref{lem:alg-extend-correct}.}
%    Let $e$ be an arc. The following hold:
%    \begin{itemize}
%        \item[i)] if $e$ is not a self-bivalent arc, then there is at most one maximal macrotig containing $e$.
%        \item[ii)] if $e$ is a self-bivalent arc, then there are at most two maximal macrotigs containing $e$ (at most one of the form $eW$ and at most one of the form $We$).
%    \end{itemize}
%    \end{lemma}
%    
%    \begin{proof}
%    For $i)$ if $e$ is cross-bivalent, by \Cref{lem:arcs-in-microtigs}, then $e$ is contained in at most two microtigs (that are macrotigs by definition): at most one of the form $W_1e$ and at most one of the form $eW_2$, by definition). If both are present, then they can be joined into a single macrotig $W_1eW_2$. Otherwise, by \Cref{lem:arcs-in-microtigs}, $e$ is contained in at most one maximal microtig (and thus a macrotig). In either case, by \Cref{lem:uniqueprotomni}, such a macrotig can be extended to a unique maximal macrotig.
%    
%    For $ii)$, since $e$ is a bivalent arc, then we can reason as above: by \Cref{lem:arcs-in-microtigs}, $e$ is contained in at most two microtigs, and thus in at most two macrotigs. Since $e$ is self-bivalent, then by definition these microtigs cannot be joined into a macrotig, but still each can be extended to a unique maximal macrotig (by \Cref{lem:uniqueprotomni}).
%    \end{proof}

\begin{theorem}[Maximal macrotigs]
\label{lem:alg-extend-correct}
The maximal macrotigs of any strongly connected graph $G$ with $n$ nodes, $m$ arcs, and arbitrary degree have total length $O(n)$, and can be computed in time $O(m)$, with \Cref{alg:maxproto}.
\end{theorem}
\begin{proof}
By \Cref{lem:maximalbigenerator}, $G$ has $O(n)$ maximal microtigs, of total length $O(n)$. By \Cref{lem:noetwiceinproto}, every maximal microtig is contained in a unique maximal macrotig (and it appears only once inside such a macrotig), and the length of each maximal macrotig is at most the sum of the lengths of its maximal microtigs; thus, we have that the total length of all maximal macrotigs is at most $O(n)$.

Using \Cref{alg:maximalbigenerator}, we can get all the $O(n)$ maximal microtigs of $G$ in time $O(m)$ (\Cref{lem:maximalbigenerator}). Once we have them, we can easily implement \Cref{alg:maxproto} in $O(m)$-time. The correctness of this algorithm is guaranteed by \Cref{lem:noetwiceinproto}.
\end{proof}

